Quantum Black Hole Entropy and Localization in Supergravity

In this thesis, we examine in detail the notion of black hole entropy in Quantum Field Theories, with a specific focus on supersymmetric black holes and the perturbative and non-perturbative quantum corrections to the classical area-law of Bekenstein-Hawking. To examine such corrections, we employ the formalism of Sen's Quantum Entropy Function where the complete quantum entropy of a supersymmetric black hole in theories of supergravity is defined as a path-integral in the near-horizon region of the black hole. Evaluation of this path-integral can then be conducted exactly using localization computation techniques. Due to the exactness of the localization argument, the results obtained in this manner are therefore formally expected to re-sum all perturbative and non-perturbative corrections to the classical area-law, and thus connect to string-theoretic predictions. We investigate such connections in detail for specific supersymmetric black holes in the hopes of strengthening a Boltzmann-type interpretation of their thermodynamic entropy as arising from the degeneracies of the microscopic gravitational constituents (the D-branes). We find that this picture holds very precisely for two types of black holes preserving four real supercharges in both four-dimensional $\mathcal{N}=8$ and $\mathcal{N}=4$ string theories and supergravities. From a broader point of view, such results can be interpreted as providing important examples where supergravity theories encode the complete low-energy dynamics of string theories and provide a consistent effective picture. Some interesting connections to the mathematical theory of modular forms and mock modular forms are also exhibited.

==> Thesis_My_Papers.tex <==
\makeatletter
\newcommand\Notefont{\normalsize}
\long\def\bibNote#1{\gdef\@bibNote{\item[]{\Notefont#1}}}
\renewenvironment{thebibliography}[1]{%
  \@xp\chapter\@xp*\@xp{\bibname}%
  \normalfont\labelsep .5em\relax
  \renewcommand\theenumiv{\arabic{enumiv}}\let\p@enumiv\@empty
  \list{\@biblabel{\theenumiv}}{\@bibNote\settowidth\labelwidth{\@biblabel{#1}}%
    \leftmargin\labelwidth \advance\leftmargin\labelsep
    \usecounter{enumiv}}%
  \sloppy \clubpenalty\@M \widowpenalty\clubpenalty
  \sfcode`\.=\@m
}{%
  \def\@noitemerr{\@latex@warning{Empty `thebibliography' environment}}%
  \endlist
}
\makeatother

\bibNote{The present work is based on the following publications:}

\renewcommand\bibname{List of Publications}
\begin{thebibliography}{100}

\bibitem[A1]{Murthy:2013xpa} 
S.~Murthy and V.~Reys, {\it {Quantum black hole entropy and the holomorphic prepotential of $\mathcal{N}\!\!\!=\!\!\!2$ supergravity}}, {\em JHEP} {\bf 1310} (2013) 099, [\href{http://xxx.lanl.gov/abs/1306.3796}{{\tt arXiv:1306.3796}}].

\bibitem[A2]{Murthy:2015yfa}
S.~Murthy and V.~Reys, {\it {Functional determinants, index theorems, and exact quantum black hole entropy}},  {\em JHEP} {\bf 1512} (2015) 028, [\href{http://arxiv.org/abs/1504.01400}{{\tt arXiv:1504.01400}}].

\bibitem[A3]{Murthy:2015zzy}
S.~Murthy and V.~Reys, {\it {Single-centered black hole microstate degeneracies from instantons in supergravity}}, {\em JHEP} {\bf 1604} (2016) 052, [\href{http://arxiv.org/abs/1512.01553}{{\tt arXiv:1512.01553}}].  
  
\bibitem[A4]{BdW-Me}
B.~de Wit and V.~Reys, {\it {Euclidean supergravity}}, in preparation.

\end{thebibliography}

\thispagestyle{empty}

